Monte Carlo Scene Search for 3D Scene Understanding

We explore how a general AI algorithm can be used for 3D scene understanding to reduce the need for training data. More exactly, we propose a modification of the Monte Carlo Tree Search (MCTS) algorithm to retrieve objects and room layouts from noisy RGB-D scans. While MCTS was developed as a game-playing algorithm, we show it can also be used for complex perception problems. Our adapted MCTS algorithm has few easy-to-tune hyperparameters and can optimise general losses. We use it to optimise the posterior probability of objects and room layout hypotheses given the RGB-D data. This results in an analysis-by-synthesis approach that explores the solution space by rendering the current solution and comparing it to the RGB-D observations. To perform this exploration even more efficiently, we propose simple changes to the standard MCTS' tree construction and exploration policy. We demonstrate our approach on the ScanNet dataset. Our method often retrieves configurations that are better than some manual annotations, especially on layouts.

==> MCSS_Algo.tex <==
\begin{algorithm}
    \caption{MCSS}\label{alg:mcss}
    \begin{algorithmic}[1]
    \myState{$iters \leftarrow$ Number of desired runs, $\hat{\calH} \leftarrow \varnothing$}
    % \myState{$N \leftarrow$ Number of desired runs}
    % \myState{$\hat{\calH} \leftarrow \varnothing$}
    \While{$iters > 0$}
        \myState{$\calN_{curr} \leftarrow \calN_{root}, \calH \leftarrow \varnothing, \calO_\comp \leftarrow \calO_\pool$}
        % \myState{$\calN_{curr} \leftarrow \calN_{root}$}\Comment{node with no object}
        % \myState{$\calH \leftarrow \varnothing$}
        % \myState{$\calO_\comp \leftarrow \calO_\pool$}
      
        \myState{$ \mathcal{C}(\calN_{curr})\leftarrow \textsc{GetChildren}(\calO_\comp)$}

        \While{True}
            \myState{$\mathcal{N}_{curr} \leftarrow \textsc{ Descend}(\mathcal{N}_{curr}, \mathcal{C}(\calN_{curr})$)}
            % \myState{$Prop_{curr} \leftarrow \calP(Node_{curr})$}
            \myState{$\calH \leftarrow \calH + \calP(\calN_{curr})$}
            
            \myState{$ \calO_\comp \leftarrow \textsc{GetProposalPool}(\calO_\pool, \calH)$}
            \myState{$ \mathcal{C}(\calN_{curr}) \leftarrow \textsc{GetChildren}(\calO_\comp,\calN_{curr})$}
        
            \If{$\mathcal{N}_{curr} \text{ is new}$}
                \myState{$\widetilde{\calH} \leftarrow \arg\max_{S} s((\textsc{OneSim}(S, \calH))$}
                
                \myState{$\textsc{UpdateNodesWithBestScore}(\widetilde{\calH})$}
                \myState{$\textsc{UpdateProposalFitnesses}(\widetilde{\calH})$}
                \If{$s(\calH) > s(\widehat{\calH})$}
                    \myState{$\widehat{\calH} \leftarrow \widetilde{\calH}$}
                \EndIf
                \myState{\textbf{break}}
            \EndIf

        \EndWhile
        \myState{$iters \leftarrow iters - 1$}
    \EndWhile
    \myState{\return $\widehat{\calH}$}
    \end{algorithmic}
\end{algorithm}

==> alg.tex <==
%%% ALGORITHM

\errorcontextlines\maxdimen

% begin vertical rule patch for algorithmicx (http://tex.stackexchange.com/questions/144840/vertical-loop-block-lines-in-algorithmicx-with-noend-option)
\makeatletter
% start with some helper code
% This is the vertical rule that is inserted
    \newcommand*{\algrule}[1][\algorithmicindent]{\makebox[#1][l]{\hspace*{.5em}\thealgruleextra\vrule height \thealgruleheight depth \thealgruledepth}}%
% its height and depth need to be adjustable
\newcommand*{\thealgruleextra}{}
\newcommand*{\thealgruleheight}{.75\baselineskip}
\newcommand*{\thealgruledepth}{.25\baselineskip}

\newcount\ALG@printindent@tempcnta
\def\ALG@printindent{%
    \ifnum \theALG@nested>0% is there anything to print
        \ifx\ALG@text\ALG@x@notext% is this an end group without any text?
            % do nothing
        \else
            \unskip
            \addvspace{-1pt}% FUDGE to make the rules line up
            % draw a rule for each indent level
            \ALG@printindent@tempcnta=1
            \loop
                \algrule[\csname ALG@ind@\the\ALG@printindent@tempcnta\endcsname]%
                \advance \ALG@printindent@tempcnta 1
            \ifnum \ALG@printindent@tempcnta<\numexpr\theALG@nested+1\relax% can't do <=, so add one to RHS and use < instead
            \repeat
        \fi
    \fi
    }%

% the following line injects our new indent handling code in place of the default spacing
\patchcmd{\ALG@doentity}{\noindent\hskip\ALG@tlm}{\ALG@printindent}{}{\errmessage{failed to patch}}
\makeatother

% the required height and depth are set by measuring the content to be shown
% this means that the content is processed twice
\newbox\statebox
\newcommand{\myState}[1]{%
    \setbox\statebox=\vbox{#1}%
    \edef\thealgruleheight{\dimexpr \the\ht\statebox+1pt\relax}%
    \edef\thealgruledepth{\dimexpr \the\dp\statebox+1pt\relax}%
    \ifdim\thealgruleheight<.75\baselineskip
        \def\thealgruleheight{\dimexpr .75\baselineskip+1pt\relax}%
    \fi
    \ifdim\thealgruledepth<.25\baselineskip
        \def\thealgruledepth{\dimexpr .25\baselineskip+1pt\relax}%
    \fi
    %\showboxdepth=100
    %\showboxbreadth=100
    %\showbox\statebox
    \State #1%
    %\State \usebox\statebox
    %\State \unvbox\statebox
    %reset in case the next command is not wrapped in \myState
    \def\thealgruleheight{\dimexpr .75\baselineskip+1pt\relax}%
    \def\thealgruledepth{\dimexpr .25\baselineskip+1pt\relax}%
}
% end vertical rule patch for algorithmicx

